Surfing: Iterative optimization over incrementally trained deep networks

We investigate a sequential optimization procedure to minimize the empirical risk functional $f_{\hat\theta}(x) = \frac{1}{2}\|G_{\hat\theta}(x) - y\|^2$ for certain families of deep networks $G_{\theta}(x)$. The approach is to optimize a sequence of objective functions that use network parameters obtained during different stages of the training process. When initialized with random parameters $\theta_0$, we show that the objective $f_{\theta_0}(x)$ is "nice'' and easy to optimize with gradient descent. As learning is carried out, we obtain a sequence of generative networks $x \mapsto G_{\theta_t}(x)$ and associated risk functions $f_{\theta_t}(x)$, where $t$ indicates a stage of stochastic gradient descent during training. Since the parameters of the network do not change by very much in each step, the surface evolves slowly and can be incrementally optimized. The algorithm is formalized and analyzed for a family of expansive networks. We call the procedure {\it surfing} since it rides along the peak of the evolving (negative) empirical risk function, starting from a smooth surface at the beginning of learning and ending with a wavy nonconvex surface after learning is complete. Experiments show how surfing can be used to find the global optimum and for compressed sensing even when direct gradient descent on the final learned network fails.

==> additional.tex <==
% !TEX root = surfing.tex

\section{Additional Simulations}
\label{sec:addsims}

Here we give additional plots for experiments comparing surfing over a sequence of networks during training to gradient descent over the final trained network. As described in the main text,
we consider the problem of minimizing the objective $f(x) = \frac{1}{2}\|G(x) - G(x_*)\|^2$, that is, recovering the image generated from a trained network $G(x) = G_{\theta_T}(x)$ with input $x_*$. We run surfing by taking a sequence of parameters $\theta_0, \theta_1,...,\theta_T$, where $\theta_0$ are the initial random parameters and the intermediate $\theta_t$'s are taken every 40 training steps. In order to improve convergence speed we use Adam \citep{kingma2014adam} to carry out gradient descent in each step in surfing. We also use Adam when optimizing over the just the final network. We apply surfing and regular Adam for 300 trials, where in each trial a randomly generated $x_*$ and initial point $x_{init}$ is chosen. Figure \ref{fig:more} shows
the distribution of the distance between the computed solution $\hat x_T$ and the truth $x_*$ for VAE, WGAN and WGAN-GP,
using surfing (red) and regular gradient descent with Adam (blue), over three different input dimensions $k$.

\begin{figure}[h]
\begin{center}
\begin{tabular}{ccc}
  \\[20pt]
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/VAEdim-20} \\
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/WGANdim-20}\\
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-5} &
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-10} &
\includegraphics[width=.3\textwidth]{newfigs/WGAN-GPdim-20}
\end{tabular}
\end{center}
\caption{Distribution of the distance between solution $\hat x_T$ and the truth $x_*$ for VAE, WGAN and WGAN-GP,
using surfing (red) and regular gradient descent with Adam (blue) over three different input dimensions $k$.}
\label{fig:more}
\end{figure}


==> newfigs/form.tex <==
\begin{table}[t!]
\begin{center}
  \vskip20pt
\begin{tabular}{|l|ccc|ccc|}
  \hline
Model           & \multicolumn{3}{c|}{VAE} & \multicolumn{3}{c|}{DCGAN} \\
\hline
Input dimension & 5       & 10    & 20    & 5       & 10      & 20     \\
Regular Adam    & 99.3    & 100   & 100   & 50.3    & 69.3    & 67.7   \\
Surfing         & 99.3     & 100   & 100   & 91.3    & 96.7    & 99.3    \\
\hline
\end{tabular}
\vskip10pt
\begin{tabular}{|l|ccc|ccc|}
  \hline
Model           & \multicolumn{3}{c|}{WGAN} & \multicolumn{3}{c|}{WGAN-GP} \\
\hline
Input dimension & 5       & 10    & 20    & 5       & 10      & 20     \\
Regular Adam    & 48.3    & 75.0  & 91.0  & 46.7    & 63.7    & 69.7   \\
Surfing         & 86.7    & 99.3  & 100   & 92.0    & 97.7    & 99.0 \\
\hline
\end{tabular}
\end{center}
\vskip5pt
\caption{Surfing compared against direct gradient descent over final trained network
for different training procedures. Shown are percentages of solutions $\hat x_T$ satisfying $\|\hat x_T - x_*\| < 0.01$.}
\label{table:prop}
\end{table}
